FogROS2-PLR: Probabilistic Latency-Reliability For Cloud Robotics

Cloud robotics enables robots to offload computationally intensive tasks to cloud servers for performance, cost, and ease of management. However, the network and cloud computing infrastructure are not designed for reliable timing guarantees, due to fluctuating Quality-of-Service (QoS). In this work, we formulate an impossibility triangle theorem for: Latency reliability, Singleton server, and Commodity hardware. The LSC theorem suggests that providing replicated servers with uncorrelated failures can exponentially reduce the probability of missing a deadline. We present FogROS2-Probabilistic Latency Reliability (PLR) that uses multiple independent network interfaces to send requests to replicated cloud servers and uses the first response back. We design routing mechanisms to discover, connect, and route through non-default network interfaces on robots. FogROS2-PLR optimizes the selection of interfaces to servers to minimize the probability of missing a deadline. We conduct a cloud-connected driving experiment with two 5G service providers, demonstrating FogROS2-PLR effectively provides smooth service quality even if one of the service providers experiences low coverage and base station handover. We use 99 Percentile (P99) latency to evaluate anomalous long-tail latency behavior. In one experiment, FogROS2-PLR improves P99 latency by up to 3.7x compared to using one service provider. We deploy FogROS2-PLR on a physical Stretch 3 robot performing an indoor human-tracking task. Even in a fully covered Wi-Fi and 5G environment, FogROS2-PLR improves the responsiveness of the robot reducing mean latency by 36% and P99 latency by 33%.

==> acks.tex <==
% \section*{Acknowledgements}

\section*{Acknowledgement}
This research was performed at the AUTOLAB at UC Berkeley in affiliation with the Berkeley AI Research (BAIR) Lab. The authors were supported in part by donations from  Bosch, Toyota Research Institute, Google, Siemens, and Autodesk and by equipment grants from PhotoNeo, NVidia, and Intuitive Surgical. The research is also supported by C3.ai Digital Transformation Institute for AI resilience. 


% This research was performed at the AUTOLab at UC Berkeley in affiliation with the Berkeley AI Research (BAIR) Lab, the CITRIS ``People and Robots'' (CPAR) Initiative, the Real-Time Intelligent Secure Execution (RISE) Lab, and by the NSF/VMware Partnership on Edge Computing Data Infrastructure (ECDI) Secure Fog Robotics Project Award 1838833. This research was supported in part by Bosch. 
% We thank our colleagues for helpful discussions and testing.

==> chapters_ft/abstract.tex <==
Cloud robotics enables robots to offload complex computational tasks to cloud servers for performance and ease of management. 
However, 
cloud compute can be costly, 
cloud services can suffer occasional downtime, and connectivity between the robot and cloud % and cloud networks 
are prone to %server outages and 
variations in network Quality-of-Service (QoS). 
We present FogROS2-FT (Fault Tolerant) to mitigate these issues by introducing
%reliance on cloud infrastructure inherently brings concerns about unpredictable cloud faults, such as server outages and server network congestion. 
% Fault tolerance is a desirable feature for safety-critical cloud robotics, yet it often comes with significant complexity and expense, posing challenges for practical deployment. 
% In our study, w
%
%We demonstrate the fault tolerance with FogROS2-Fault Tolerance (FT), adding
a multi-cloud extension that automatically replicates independent stateless robotic services% on low-cost spot Virtual machines
, routes requests to these replicas, and directs the first response back. With replication, robots can still benefit from cloud computations even when a cloud service provider is down or there is low QoS.  Additionally, many cloud computing providers offer low-cost ``spot'' computing instances that may shutdown unpredictably. Normally, these low-cost instances would be inappropriate for cloud robotics, but the fault tolerance nature of FogROS2-FT allows them to be used reliably. 
% The fault tolerant layer can be reliably deployed 
% on top of cheaper but less reliable cloud machines to reduce the deployment cost.
% \algname transparently proxies the ROS2 communication and select the first response of the fault tolerant replicated. 
% With doubled the fault tolerance, \algname achieves a 30\% cost reduction to conventional cloud robotics and X times cost reduction to fault tolerant environment on a physical pick-and-place manipulation task. 
We demonstrate FogROS2-FT fault tolerance capabilities in 3 cloud-robotics scenarios in simulation (visual object detection, semantic segmentation, motion planning)
% and physical pick-scan-place. \nan{suggestion: a physical robot experiment: scan-pick-n-place}
and 1 physical robot experiment (scan-pick-and-place).
Running on the same hardware specification,  
\algname achieves motion planning with up to 2.2x cost reduction and up to a 5.53x reduction on 99 Percentile (P99) long-tail latency.
\algname reduces the P99 long-tail latency of object detection and semantic segmentation by  2.0x and 2.1x, respectively, under network slowdown and resource contention. 
% \eric{we want to emphasize that FT is strong at minimizing latency for the long runs/long tail events, don't know if thiss a clear way to say it}. \trinity{p99 is pretty standard and tails significantly impact p99 so I think this is a good measurement}
Videos and code are available at 
\url{https://sites.google.com/view/fogros2-ft}.
% \eric{schochatii for network and compute time, faster responses }

==> chapters_ft/design.tex <==


\section{\algname Design}
%In this section, we answer two main questions: (1) How does \algname achieve fault tolerance that is transparent to ROS2 applications? (2) How does \algname resiliently maintain a pool of cost-efficient cloud servers? 
This section describes how \algname (1) achieves transparent fault tolerance for ROS2 applications and (2) resiliently maintains a pool of cost-effective cloud servers.


\subsection{Overview}
Figures \ref{fig:design:overview} show an overview of how \algname achieves both fault tolerance and cost effectiveness. \algname sends requests to multiple replicated spot VMs, and routes the first response back to the robot. It resiliently manages spot VMs to  recover from unpredictable terminations.   
% \jeff{Also provide an overview description here, and refer back to the figure as appropriate }

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/overview.png}
    \caption{\textbf{System Overview of \algname}  \algname transparently proxies ROS2 communication. It sends requests to multiple replicated spot VMs, and routes the first response back to the robot. \algname manages spot VMs to resiliently recover from unpredictable terminations. }
    \label{fig:design:overview}
\end{figure}


\textbf{Interface}.
A user interfaces to \algname is through extensions to the ROS2 launch system.
The interface is identical to standard ROS2 launch scripts, other than specifying the hardware requirements and desired fault tolerance level.
Listing \ref{lst:launch} shows an example of a launch script for fault tolerant grasp planning service with \algname. 
We embrace the Sky \cite{chasins2022sky} multi-cloud paradigm
%\jeff{Sky needs a definition and citationg}
that user can directly specify generic hardware requirements instead of specific cloud machine types, which are compatible across heterogeneous cloud service providers. 

\begin{listing}[t]
\inputminted[xleftmargin=20pt,linenos,fontsize=\scriptsize,escapeinside=||]{python}{listing/launch_example.py}%
% \begin{tikzpicture}[remember picture, overlay]
%   \node [fit=(pic cs:machinestart)(pic cs:machineend),inner xsep=2pt, inner ysep=6pt, xshift=-1pt, yshift=2pt, rounded corners,draw=black] {};
%   \node [fit=(pic cs:attrstart)(pic cs:attrend),inner xsep=2pt, inner ysep=6pt, xshift=-1pt, yshift=2pt, rounded corners,draw=black] {};
% \end{tikzpicture}%
% \vspace{-12pt}
\caption{\textbf{\algname Launch Script Example.}  This example launches two nodes, a grasp motion client node that runs locally with standard ROS2 interface, and a fault tolerant grasp planning node with \algname. It allow users to specify the cloud ROS2 nodes and desired fault tolerance level and hardware with mixed on-demand and spot VMs. } 
\label{lst:launch}
\end{listing}



\subsection{Application-Agnostic Fault Tolerance through Replication}

% \eric{explain a few problems: 
% 1. how routers figure out the request-response workflow 
% 2. tree construction and row out through bfs 
% 3. on request, ; on response, 
% }

%To enable the seamless integration of unmodified ROS2 applications, 
To launch (unmodified) ROS2 nodes in the cloud,
\algname 
%is designed as \jeff{``is designed as'' is a ambiguous (and also passive voice), can we change it to `uses' or `integrates' or just `is'?}
is a \textit{multi-cloud launcher} that facilitates cloud initialization  and \textit{a replication-aware proxy} that connects ROS2 robot client and cloud service with a global fault-tolerant network. 

The multi-cloud launcher initializes cloud servers with a ROS2 environment, and provisions secure communication through \algname \emph{proxies}. 
To local ROS2 network, the proxy serves the requests as local ROS2 service and interacts with nodes (e.g., sensors and controllers) on the robot as if the ROS2 service nodes on the cloud were all on the same local computer.
On a new request, the proxy of \algname sends the request to all replicated service nodes. When the proxy receives responses from the replicas, it passes only the first response to the robot. This is agnostic to applications and causes of the fault. As long as one response comes back to the robot, the request is fulfilled. To the cloud server, the proxy receives the request from the network, and invokes the ROS2 service on the cloud. 

\textbf{Multi-Cloud Fault Tolerant Launching Process}.
Initializing fault tolerant cloud robotics includes the following steps (1) The robot provisions multiple Cloud servers across different regions and data centers. \algname can automatically select the region based on network latency and cloud operating cost. The user can override the selection with configuration. \algname uses SkyPilot~\cite{yang2023skypilot} to interface with heterogeneous cloud service providers. (2) The robot initializes all the cloud servers with ROS2 and the robot service application dependencies. FogROS2~\cite{ichnowski2022fogros} details the initialization procedure. (3) Robot and all Cloud servers generate and share communication security credentials (4) Robot and all Cloud servers run \algname proxy 
% \jeff{why do cloud servers run the proxy? In the previous paragraph, the proxy was only for replicating requests. Is this so that clouds can request against each other? If so, neat! Let's make that explicit.} 
(5) All proxies discover each other automatically, establish global and resilient connectivity with the generated security credentials and desired topology. 

By default, all robotics services 
% \jeff{what's a service? is it a node?}
have at least two replicas at different cloud data centers.
% Note: do not use ``Safety-critical'' here---it has specific meaning and is asking for a poke in the eye from, especially, real-time community. (Specific meaning: if a safety-critical system fails it may injure or harm a human. I don't think we should make the argument that one should run safety-critical things on FogROS2-FT) -JI
Critical services can use more replicas and adapt based on changing conditions (such as time of the day, budget). Without terminating the existing cluster, one can use Command Line Interface (CLI) to scale up and down the number of replicas dynamically:
\[
\texttt{\footnotesize ros2 fog scale [up/down] [args]}
\]

% \jeff{Can you provide a better example of why one would change the scaling dynamically? I would think criticality of a service would be known upfront, and thus go in the launch file.  Perhaps, an argument could be made that its for adapting to changing conditions..., but not sure what conditions those would be.} %\trinity{from Christian J: ``clarify, does this work during runtime?"}

% \jeff{If CLI is post-launch, I seems better to go after the next section. It flows more logically that way.  (A) how to specify what to launch, (b) how FogROS2-FT launches, (C) CLI to update things after launch.}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/flow.png}
    \caption{\textbf{Flow diagram of \algname on handling new requests} %This provides a high-level overview of how 
    The \algname replication-aware proxy handles ROS2 grasp planning request with fault tolerance guarantees with multiple steps. (1) The ROS2 application sends a request on the local ROS2 network.
(2) The proxy running on the robot receives the request and extracts the content and a unique identifier %from raw buffer 
from ROS2 middleware (rmw) layer buffer. 
(3) The proxy registers the unique ID from rmw with the \textit{handle}, which includes a callback function if the response of the request arrives and a callback function for timeout.
(4) The proxy securely sends the request to proxies running on replicated Cloud machines. %The proxies are connected peer-to-peer, so t
There can be multiple proxy hops between the robot and the server that hosts the desired ROS2 service. 
The request message carries the unique identifier and the proxy adds an entry in the registry table.
(5) The proxy running on the cloud converts the message to a standard ROS2 request message, and invokes the ROS2 service on the cloud and gets the response. 
%By ROS2 service implementation, the response messages keeps the same unique identifier as the request message. 
(6) The proxy on the cloud sends the response back to the proxy on the robot. % with the same path.
(7.A) The robot checks if it handled the response %is handled 
with the unique identifier; % and marks the request as fulfilled;
(7.B On the duplicated responses) The proxy drops the response if it was already handled. %the response associated with the identifier is handled. 
(7.C On timeout) The proxy calls the timeout handler (such as returns with empty response) and cleans up the registry table.
(8) The robot sends the response to the application on the robot through standard ROS2 protocol. 
}
    \label{fig:design:flow}
\end{figure}

\textbf{Replication-Aware Fault Tolerant Connectivity}.
Figure \ref{fig:design:flow} shows the workflow of \algname on handling requests with fault tolerance.  A ROS2 application sends a request via the local ROS2 network, where the robot's proxy captures, extracts its serialized content a unique identifier from the ROS2 middleware layer (rmw). The proxy stores the identifier with a \textit{handle} and sends the request to the cloud. The handle incorporates a callback function called on response arrival and on timeout. The cloud proxy invokes the corresponding cloud-based ROS2 service to compute and send the response back. The robot's proxy verifies the response with the unique identifier, then either marks the request as completed and sends back to the robot, or discards as a duplicate.
% \ken{move (1)-(8) to Fig. 3 to avoid duplication?} \eric{fixed but it seems to be too long? }
%\eric{will fix it, but I do think this is important, and I prefer to put in the main text and keep the caption concise (?) }

% The original FogROS2-SGC uses this property for mobility, allowing robots to move freely across different network domains. \algname extends \sgc's identifier generation process so that multiple servers at various geographic locations can host the same ROS2 service by assigning their service interfaces with the same identifier. 
% \algname also supports identifier generation for both ROS2 publish/subscribe and service/client communication paradigm.  


\subsection{Resilient and Flexible Connectivity}
The fault tolerance workflow of \algname is established on a global peer-to-peer network, a fabric formed by interconnected proxies. The connections are resilient to service changes and flexible to various network topologies. 

% \textbf{Resilient Connectivity}.
When a cloud machine is interrupted and rebooted, \algname launches another cloud virtual machine. The launched cloud machine is typically different cloud machine with changed network connectivity information (such as IP address). 
The connections between proxies should be resilient to such interruption that even if the server gets interrupted and relaunched at a different physical machine, it can still maintain its connection to the robot. 

\algname achieves this by assigning a globally unique identifier to every peer-to-peer connection between proxies. 
This identifier can be generated deterministically between the proxies that no other ROS2 service can produce the same identifier. \sgc~\cite{chen2023sgc} provides details about the identifier construction process and guarantees.  
%provides details about the cryptographic \jeff{first mention of `cryptographic,' a reader unfamiliar with SGC may be confused. either discuss the unique itentifier as cryptographic from the start, or motivate the cryptographic process here} construction process, 
% which the collision \jeff{reader is unlikely to know what `collision' refers to. its probably okay to drop this part of the discussion.} is practically impossible for large identifier space. 
In this work, we extend the identifier of \sgc to network connections, such that even if the original machine is interrupted and restarted at a different place, it can still deterministically generate the identifier and resume the connectivity. 
\algname connects the proxies on the robot and on the cloud with the same globally unique identifier by a metadata server. The metadata server exchanges network information, monitors the status of the connections, and cleans up the connectivity information if one of the proxy reports its peer as disconnected. The metadata server can be hosted on lightweight, low-bandwidth and accessible cloud servers. The server is only used for connectivity establishment, and no application data flows through the server, so the failure of the server does not lead to a system failure. %\jeff{does the server then become a single point of failure?} 

\textbf{Flexible and Scalable Topology For Bandwidth-Limited Robots}.
We consider mobile robots with low network bandwidth that may be bottlenecked if sending the request to multiple cloud servers. In this case, we need an intermediate server with higher bandwidth as gateway to forward the requests to other proxies. The server can be on the cloud or edge.
The transport of \algname is not constrained to having the client and server be directly connected. In \algname, the proxy can be in a tree-like structure, where each edge the tree connects between an intermediate hop and the proxy. The proxy finds and establishes connections with its peers by flattening the tree with Breadth-First-Search (BFS). Figure \ref{fig:mcast}\,(b) shows two possible topology examples, which one can launch a lightweight gateway server to facilitate the message replication, or directly use a proxy on the compute service node. %For each link, \algname constructs different connectivity channels associated with a globally unique name. % \jeff{$\leftarrow$ something is missing from the previous sentence, it doesn't read clearly}. 

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/mcast.png}
    \caption{\textbf{Flexible Topology for Different Bandwidth of Robots} \textbf{(a)} Since \algname sends replicated requests to multiple cloud machines, it demands more network bandwidth than conventional cloud-robotics deployments. \textbf{(b)} \algname allows flexible topology so that low-bandwidth robot can leverage cloud machines with higher bandwidth to forward to replicated services. One can either use dedicated gateway machine (left) or existing compute servers (right). }
    \label{fig:mcast}
\end{figure}



\subsection{Resilient and Cost-Efficient Spot VMs}
% Spot VM
\algname %\jeff{can use? (e.g., one option of may)} 
can use spot VMs to reduce the cost of the replicated cloud server deployment. %Spot VM is a special pricing model that offers the same server types and performance as typical compute servers, but can reduce the compute resource cost up to 90\%. As a result, 
Since spot VMs can be up 90\,\% lower cost than their equivalent on-demand VMs,
running two spot VMs at the same time can still enjoy as much as 80\,\% cost reduction. % assuming 90\,\% discount compared to running one traditional cloud server. 
%However, these spot VM servers might be terminated and reclaimed at any time by the cloud service providers. 
Earlier studies~\cite{10.1145/3458336.3465301} show a bioinformatics task with 24 spot VMs on Google Cloud Platform experiences a preemption every 36 minutes on average. 
Because of the fault tolerance extension of FogROS2, we are able to guarantee per-request availability that as long as there is one spot VM not preempted and available to serve the request. 
\algname launches and manages spot VMs across multiple cloud service providers and regions. 
% \jeff{Shouldn't the paper mention SkyPilot in the previous subsection? Or does \algname only use SkyPilot spot VMs. If so, this should be explained.}
\algname regularly monitors the status of the spot VMs. When a spot VM is interrupted, \algname re-launch the service node on a new spot VM and re-establishes connectivity. 


% \begin{figure*}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/efficiency.png}
%     \caption{\textbf{Overview of \algname Fault Tolerance Layer} \eric{likely leave this to future}}
%     \label{fig:design:overview}
% \end{figure*}



% \subsection{Memory and Compute Efficient Request Management} 
% \eric{this depends on how much we have for the experiment section } \eric{okay this subsection goes to another system paper}

% \textbf{Threading Model for efficient request-response management}
% In order to increase the throughput and application responsiveness, \algname needs to be asynchronous, meaning that it is able to continue receiving, processing and forwarding messages without being blocked by prior requests. It becomes challenging to efficiently keep track of all the unprocessed requests. In the proxy of \algname, we develop an efficient threading model for managing all the requests and responses, and a memory model to efficiently pass the request and response buffers across threads. 


% %Robots with few CPU cores usually have low network performance because network operations are usually \textit{blocking}, where the entire packet processing halts and waits for the network operations to finish. \algname improves CPU utilization by leveraging asynchronous Rust interfaces~\cite{tokio}. Asynchronous interfaces are non-blocking, removing the network operations out of  critical path of message processing. 
% % In this architecture, every connection is assigned to a lightweight asynchronous thread. Instead of blocking or waiting for the network operation to complete, other lightweight threads continue to process other messages while waiting. Multiple network operations can be handled at the same time without blocking and waiting. The framework is event-driven that the threads only run if there are new messages to process. This prevent wasting compute resources while waiting for new messages.


% \textbf{Memory Model for buffer management}
% Because the threading model requires the messages to pass from one thread to another, \algname eliminates memory copying operations and the need for synchronization when passing the message buffers.
% As a result, the networking transport component of \algname is implemented with Rust\ken{add to abstract}, a programming language that features a single ownership model: every data object has a single owner, and passing the data is moving the ownership from one variable to another. \algname maintains a heap of message buffers that stores the actual objects. When replicating the requests and sending to multiple replicas, only the reference of the message buffer object is copied to the thread that responsible for sending the message, while the actual request message buffer on the heap does not involve any copying relationship. 



==> chapters_ft/eval.tex <==

% \section{Cloud Robotics Evaluation}
% \section{Single-Server vs. \algname Experiments}
% \jeff{Can we call this section just `Experiments'? I started looking for other differently qualified Experiment sections...}

\section{Experiments}

\subsection{Setup}
Without modifying the application code, we apply \algname to three cloud robotics applications: visual object detection with YOLOv8~\cite{redmon2015you}, Semantic Segmentation with Segment Anything~\cite{kirillov2023segment} and motion planning with Motion Planning Templates (MPT)~\cite{ichnowski2019mpt}. 
% We demonstrate that with \algname, we can analyze the trade-offs between heterogeneous applications. % \ken{omit}
We use SkyPilot \cite{yang2023skypilot} to select servers given a hardware specification. % and to query  the hourly cost. % \ken{omit}
For all the experiments, we use Amazon Web Services (AWS) spot VMs with two replicas in different regions, us-west-1 (California) and us-west-2 (Oregon).

\textbf{Metrics}.
We compare \algname with baseline single-server deployment by average latency collected by 100 trials for motion planning and 300 trials for robot vision tasks. We quantify \textit{long-tail} anomalous latency faults with 99 Percentile (P99) latency, the runs with the top 1\,\% latency. 

\textbf{Cloud Cost} 
Table \ref{tab:eval:cost} shows the US\$ per hour cost of \algname compared to typical cloud robotics single-server setup. With Spot VMs, \algname is up to 2.13x cheaper than conventional single-server cloud robotics setup.
\input{tables/cost}

\subsection{Case Study: Parallel Motion Planning}
We perform a latency analysis of \algname for parallel motion planning tasks on 3 different scenarios of varying complexity provided by Open Motion Planning Library (OMPL)~\cite{OMPL}. Given a robot's initial state and goal state, motion planner computes the waypoints required to move the robot to the goal while avoiding the obstacles. The motion planning algorithms we test are iterative optimization problems with stochastic solve times.% depending on how close the randomized initial plan is to the optimal solution.

\begin{figure}
    \centering
    
    \includegraphics[width=\linewidth]{figures/mp_results.pdf}
    \caption{\textbf{\algname Latency on Motion Planning Template} We tested \algname on 3 different motion planning environments (columns (a), (b), and (c)). Due to the stochastic nature of the algorithm, we aggregated results for each scenario and server configuration over 100 trials with a 100\,s timeout. The \textbf{(top row)} %For each scenario, the \textbf{top image}
    shows the frequency histogram for the scenario when {run} with Single-Server (in blue).
    The \textbf{(middle row)} shows the frequency histogram for the scenarios when run on 2 servers with \algname (in orange). With all scenarios, the shift left of \algname histograms (in orange) relative to their corresponding single-server histograms (in blue) indicates improved latency performance when running on replicated servers. The \textbf{(bottom row)} compares the cumulative distribution functions (CDF) for single-server (in blue) and two servers (in orange). The two-server CDF is left relative to the single-server CDF indicating an overall improved performance with lower average latency for all scenarios. } 
    \label{fig:eval:mpt}
\end{figure}
% \textbf{Experiment Setup}
% Under normal circumstances, only 1 server is attempted to compute the motion plan from a given request. However, because of the redundancy offered by \algname, at least 2 servers are running to solve the motion planning task to solve a given request. Thus, for 4 motion planning tasks,

\textbf{Latency Analysis}
We compare the latency probability between single-server and \algname with 2 servers in Fig. \ref{fig:eval:mpt}.
The results for the motion planning latency analysis are summarized in Figure~\ref{fig:eval:mpt}. For all 3 scenarios, \algname reduces average latency by up to 1.22x on Cubicles. \algname significantly mitigates anomalous long and randomized latency by 1.42x (TwistyCool) and 5.53x (Cubicles) on P99 long-tail latency, because the probability of simultaneous anomalous high latency is rare. 

\input{tables/mpt_cost}

% \begin{figure}
%     \centering
    
%     \includegraphics[width=\linewidth]{figures/mpt_results.png}
%     \caption{\textbf{\algname on Motion Planning Template} \algname was tested on 4 different motion planning environments. Due to the stochastic nature of motion planning, each scenario for each server configuration was run for 100 trials. The x-axis for all graphs is latency in milliseconds. For each subfigure, the \textbf{top image} shows the frequency histogram for the scenario when {run} with single-server (in blue). The \textbf{middle image} shows the frequency histogram for the scenario when run with two servers (in orange). With all 4 scenarios, the two server histograms (in orange) are all skewed to the left relative to their corresponding single-server histograms (in blue) indicating improved latency performance when the motion planning scenario is run on 2 servers. The \textbf{bottom image} compares the cumulative distribution functions for single-server (in blue) and two servers (in orange). The two server CDF is left relative to the single-server CDF indicating an overall improved performance with lower average latency for all 4 scenarios. \eric{a better way of presenting these figures?}\ken{for (c) Apartment, can we show with higher Pserver(failure)?} \eric{@Kush, how to address this issue, also I tend to make it 4 x 3 to save some space}} \kush{Worried that making it 4x3 will make the figures too small?}
%     \label{fig:eval:mpt}
% \end{figure}



\subsection{Case Study: Robot Vision with YOLOv8 and SAM}
% \ken{Case Study: YOLOv8 Robot Vision} \eric{we also have SAM}


% \begin{figure}
%     \centering
%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/sam-cdf.pdf}
%     \end{subfigure}%
%     \\
%     \begin{subfigure}{0.6\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/sam-histogram.pdf}
%     \end{subfigure}
%     \caption{\textbf{\algname on Semantic Segmentation with SAM under Compute Resource Oversubscription}  \algname improves 30\% of the long-tail P99 latency for SAM. 
%     As cloud GPU resources are typically oversubscribed and shared by multiple concurrent clients, we emulate such resource contention by running another periodic and concurrent client that alternates to send requests to \algname server. On each server. \algname significantly reduces the long-tail latency caused by the resource contention by 1.96 times. }
%     \label{fig:eval:sam}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/sam_results.pdf}
    \caption{\textbf{\algname on Semantic Segmentation with SAM under Faults (F) by Compute Resource Oversubscription}  \algname improves 30\,\% of the long-tail P99 latency for SAM. 
    As cloud GPU resources are typically oversubscribed and shared by multiple concurrent clients, we emulate such resource contention by running another periodic and concurrent client that alternates to send requests to \algname server. \algname significantly reduces the long-tail latency caused by the resource contention by 1.96x. }
    \label{fig:eval:sam}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/yolo_results.pdf}
    \caption{\textbf{\algname on Object Detection with YOLOv8 under Faults (F) by Regional Network Slowdown} 
    We use \algname to launch a multi-cloud cluster that includes us-west-1 (California) and us-west-2 (Oregon).
    \algname and single-server deployments demonstrates similar latency under good network conditions, as the additional latency of sending to another replicated service is amortized \algname using the first response. 
    To simulate network congestion that can occur when a robot has trouble connecting to a specific data center,
    we introduce 100\,ms latency on all our servers in us-west-1 (labeled with (F) for `fault'). With the network slowdown, \algname is 2.1x faster on average than non-fault tolerant deployment, and 3.9x faster on P99 latency.}
    \label{eval:yolo:results}
\end{figure}


% \begin{figure}
%     \centering
%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/yolo-cdf.pdf}
%         % \caption{Latency CDF for YOLO}
%     \end{subfigure}%
%     \\
%     \begin{subfigure}{0.6\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/yolo-histogram.pdf}
%         % \caption{Latency Histogram for YOLO}
%     \end{subfigure}
%     \caption{\textbf{\algname on Object Detection with YOLOv8 under Regional Network Slowdown} 
%     We use \algname to launch a multi-cloud cluster that spans across US-west-1 and US-west-2.
%     \algname demonstrates similar latency when no additional latency is introduced, as the additional latency of sending to another replicated service is amortized by the ability to take the first response. 
%     Network congestion occurs if the robot has trouble connecting to a specific data center. 
%     We introduce 100ms latency on all our servers at US-west-1. In the light of network slowdown, \algname is 2.1x faster on average than non-fault tolerant deployment, and 3.9x faster on P99 latency.}
%     \label{eval:yolo:results}
% \end{figure}

We evaluate \algname with SAM and YOLOv8. SAM is a computationally expensive algorithm that requires long computational time even with GPU. The result in Fig. \ref{fig:eval:sam} (Single-Server) shows the latency of running SAM on a typical setup with one cloud server, SAM shows a long-tail and significant P99 latency. \algname improves the P99 latency by 1.3x by selecting the first response from the duplicated services. 
Compared to SAM, YOLO has lower inference latency, thus more network-intensive. 
In this case, \algname demonstrates similar latency as Single-Server deployment for the tradeoff that \algname consumes more network bandwidth but the additional latency is amortized by more stable response time.

\textbf{Faults at Compute Resource Oversubscription} 
We evaluate \algname against the faults of resource contention if many robots are contending on few resources, where one may choose to run multiple services on the same physical machine. By comparing faults (F) between Single-Server (F) and \algname (F) in Fig.\,\ref{fig:eval:sam}, \algname reduces the latency by 1.31x and long-tail P99 latency by 1.96x. 

\textbf{Faults at Regional Network Slowdown}. 
Sometimes robot may experience slowdown when connecting to a specific cloud data center. This can be caused by a periodic and regional network congestion or physical location. By comparing faults (F) between Single-Server (F) and \algname (F) in Fig.\,\ref{eval:yolo:results}, \algname reduces the latency by 2.1x and long-tail P99 latency by 3.9x. 

\subsection{Case Study: Physical Scan-Pick-and-Place}
% \eric{following proposal from Nan@Bosch as placeholder}

% \begin{figure}
%     \centering
%     % \begin{subfigure}{0.6\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/physical_setup_1.png}
%         \caption{\textbf{System Diagram and Physical Setup:}(Left)(Right)}
%         \label{fig:eval:pnp:setup}
% \end{figure}

\begin{figure}
    \centering
        \centering
        \includegraphics[width=\linewidth]{figures/physical_eval_setup.png}
        \caption{\textbf{Physical Setup and System Diagram.} \textbf{(Left)} In the scan-pick-and-place robotic task, the goal is to move an object from one workspace to a randomly generated location on the other workspace.  We repeat the task (from left to right, from right to left) for hours to show the continuity and robustness of \algname in a physical robot system. \textbf{(Right)} The system diagram has two spot VMs providing Apriltag localization services to a UR10e robot with a RealSense Camera mounted on its wrist. The robot and camera connect to an edge computer that runs a robot motion planner and a \algname proxy to connect to the replicated cloud services.}
        \label{fig:eval:pnp:setup}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{figures/apriltag_kill.pdf}
    \caption{\textbf{\algname on Physical Fault Tolerant Pick-Scan-Place} (A) \algname achieves reliable latency by choosing the first response with two active servers (B) We manually terminate one spot VM to emulate a fault, and \algname uses the responses from spot VM \#2. (C) \algname automatically recovers spot VM \#1 from failure by re-initializing user's environment and connectivity (D) We terminated spot VM \#2 to emulate spot VM preemption (E) \algname recovers and uses responses from both servers. %The failed spot VMs are recovered from a generic Ubuntu image. <-- seems unintersting to reader. -JI
    The recovery downtime can be improved by tools from FogROS2~\cite{ichnowski2022fogros}.}
    \label{fig:eval:physical:result}
\end{figure}

We evaluate \algname with cloud-based scan-pick-and-place with a fundamental physical robotic skill for many robot tasks, such as random bin picking, sorting, kitting, and conveyor belt pick-n-place. 
By offloading visual perception services, \algname improves the responsiveness and reliability in spite of faults.

% \nan{ In factory automation and warehouse logistics, to visually localize an object and then perform pick-n-place, or scan-pick-n-place, is a fundamental physical robotic skill that is required for many robot tasks, such as random bin picking, sorting, kitting, and conveyor belt pick-n-place.  By off-loading visual perception services to the Cloud, one can dramatically reduce the hardware costs of local perception servers.  However, the reliability of Cloud services has always been in question to support long-running continuous operations in factories. 
% \\
% \\
% Via physical robotics pick-n-place experiments, we demonstrate that \algname hosting redundant perception services in spot instances can improve reliability and responsiveness, and reduce the operation cost of the scan-pick-n-place, compared to single instance Cloud service.  Hence, it is better to use \algname for factory robot deployments due to its reliability and lower costs.}

\textbf{Experiment Setup}
Fig. \ref{fig:eval:pnp:setup} shows the physical setup of the Scan-Pick-and-Place evaluation. 
The Universal Robots arm (UR10e) is mounted with an Intel RealSense D435i on the wrist. 
We use a suction gripper to grasp a plastic CD player marked with an Apriltag. 
The system executes a cyclical procedure that begins with the robot moving to a predefined joint position. 
We implement a perception ROS2 service that 
 uses Apriltag~\cite{wang2016apriltag} for pose estimation.
% Then, the camera captures a monocular image at 640x480 resolution, and dispatches the camera info and compressed image to the cloud as a ROS2 service request via
The ROS2 service takes in 640x480 resolution image frames and returns a 6D pose of the target, and the robot picking motion is generated and executed with the MoveIt2 motion planning tool on the edge computer, completing the feedback loop. 
The robot arm alternate to pick-and-place a box between the left section and the right section of a designated platform.

% \jeff{The above setup sounds a little strange---apriltags are fast, so why use a cloud service for it?  motion planning can be slow, so why not use a cloud service. Also, there is a lot of passive-voice in it.}


\textbf{Latency Analysis} 
We conducted the scan-pick-and-place repeatedly and manually interrupt the spot VMs to demonstrate the robustness of the system.
Fig.\,\ref{fig:eval:physical:result} shows the latency timeline of \algname on Physical Fault Tolerant Pick-Scan-Place. We manually terminated one of the two spot instances (scenario B and D). 
There are two takeaways: (1) \algname can achieve reliable latency by choosing the first response with two active servers  (2) \algname can recover from server failures, such as termination. 
As long as one of the services is available and responsive, it can provide continuous operation for latency-sensitive applications. 




==> chapters_ft/future_work.tex <==

\section{Conclusion}
% \jeff{Change this to a `Conclusion' section. Then break into two paragraphs. first paragraph = conclusion---what the paper did/showed/described. second paragraph, start with "In future work, ..." then discuss solutions to limitations.}

In this work, we explore concurrent execution across identical and stateless service deployments on different cloud machines with \algname, and use the first received response to achieve the tolerance against independent faults. Evaluation shows \algname can reduce the long-tail latency by up to 5.53 times. 
It can be deployed on cost-efficient spot VMs that the fault tolerant system can be up to 2.1x cheaper than conventional cloud robotics setup.
% We proposed various designs to reduce the overhead of replicating the request to multiple services. 

In future work, we will use multi-path connection, for example, having mobile robot to use 5G cellular connection, Wi-Fi and Ethernet connection simultaneously to avoid failures on single network connection. This resolves the assumption of \algname that servers and faults to be independent and prevents the same network link between robot and cloud to be the single point of failure. 


% \section*{Acknowledgement}


%However, current cloud service providers do not provide hardware level multicast, so we cannot further reduce the overhead of sending to multiple servers. 
% We also assume the tasks are stateless. \algname provides a stateful storage for objects that can be recovered even if spot VMs are interrupted. However, saving the states cannot be transparent to the application, thus requires special handling from developers to use this feature as ROS2 does not provide an object storage interface.  




% We acknowledge a potential tradeoff between fault tolerance and increased application latency \jeff{unclear that we did actually...}. 




==> chapters_ft/introduction_v0.tex <==
% \eric{intro+related work 2 pages, design 2 pages, eval 2 pages, conclusion+references 2 pages}
% \eric{alternative names: 
% FogROS2-SPOT: Server-based Parallel Operations for fault Tolerance; 
% FogROS2-CRAFT: Cloud Robotics With Cost-Reduced And Fault-Tolerant Replicated Servers; 
% CARE - Cloud fAult-tolerant Replicated sErvers; or just FogROS2-FT }
\section{Introduction}
% \eric{cloud robotics reduce cost, enhance performance, ease of management by orchestrating all the computation to a centralized server}
Cloud robotics enables robots to access shared resources and services on-demand with boosted performance and simplified management. More sophisticated algorithms, such as \eric{}, can be deployed on robots without the need for powerful on-board hardware, such as GPU, TPU, and high performance CPU.
In previous research, we developed FogROS2, which enables unmodified robotics code in Robot Operating System 2 (ROS2) to offload heavy computing modules to on-demand cloud hardware resources and accelerators. 
In this work, we introduce a fault-tolerant extension to FogROS2~\cite{ichnowski2022fogros} that is more cost-efficient than previous systems while simultaneously having more robust performance. \jeff{Let's figure out if we want to motivate primarily as a fault-tolerant system or a cost-efficiency system. I propose motivating primarily around fault tolerance will be more impactful (it's probably the main objection we've seen in prior reviewer's comments), but then adding `we also get cost savings' is a surprising bonus} \trinity{agreed; In this work, we introduce a fault-tolerant extension to FogROS2~\cite{ichnowski2022fogros} that is more robust to potential disruptions and has the added benefit of cost-efficiency.}

% \eric{However, cloud introduces factor of unreliablitiy. Traditionally when a robot's compute is broken, but regional network congestions and downtime may affect all the robots, thus affecting the entire operation. The breakdown of the computational service leads to as little as latency disturbances to safety-critical. }
 
% However, the shift towards cloud computing raises issues for the reliability of long-running, safety-critical tasks. In traditional setups, a failure in a single robot's computing resources has limited, localized effects. In contrast, cloud computing introduces vulnerabilities not present in onboard computing systems, such as regional network congestion and server outages, which can impact the operations of an entire fleet of robots. This vulnerability may lead to misconceptions that  cloud robotics are not suitable for safety-critical and long-duration operations.


% \eric{Fault tolerance becomes a requirement for cloud robotics to ensure the reliable task of every request.  however, there are a few factors that makes this challenging. (1) costly by replication, (2) hard to deploy, require engineering}
Fault tolerance allows cloud-robotics tasks to continue operating effectively despite failures in cloud or network components, ensuring the necessary reliability for processing every request. \jeff{`Every' is over promising. I suggest that we should shift the focus (and introduce the robotics audience to) the notion of uptime/downtime ratios and even perhaps SLAs (e.g., \url{https://aws.amazon.com/compute/sla/}).} \eric{help think about (equation), oh cloud would be down}
Achieving such resilience, however, presents notable challenges: as it typically demands an in-depth understanding of the algorithm and specific adaptations for fault resistance, and it involves complex deployment and management processes that require extensive engineering expertise. 
Thus, there can be a misconception that cloud robotics are not suitable for long duration operations. 
%In this work, we recognize the fact that a failure in non-cloud robot systems is fatal; in contrast, 
However, cloud computing can provide redundancy and thus be more reliable, even though cloud networks are more prone to \jeff{Let's avoid using `prone to', we don't want to give the reader the impression that the cloud is worse than it is---that might leave them with the impression that they should avoid the cloud.} regional network congestion and server outages \jeff{Let's see if we can find historical data on actual outages/uptime rates.}. \algname provides fault tolerance for heterogeneous stateless robotic algorithms without requiring ROS2 application modifications. It simultaneously dispatches requests to identical services deployed in multiple cloud data centers and uses the first response received from the replicated services. This model \eric{significantly increases the probability of getting a} timely \jeff{`timely` sounds like its overpromsing too. e.g., all services are slow means it will be slow (but still faster than the slowest). Is there another wording?} responses as long as at least one replica and network remains operational.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/use_case.png}
    \caption{\textbf{\algname} Cloud robotics applications such as grasp planning, are typically deployed on a single typical cloud server, which subjects to single point of failure. Without any ROS2 application modifications, \algname is more cost-efficient than conventional cloud servers launched with FogROS2, and can be fault tolerant to individual server termination or slowdown. }
    \label{fig:intro:use_case}
\end{figure}


% \eric{specifically use replication to for fault tolerance, which further leads to following challenges: (1) ROS2 programming model does not consider replication (2) replicating and dispatching requests across replicas become computationally expensive, }
 
We design a routing network that connects a robot with a scalable number of replicated services, and filters replicated response once the request is handled. The routing network allows resilient and location independent connectivity that persists even if started on a different machine. We propose a compute-efficient threading model for asynchronously processing the requests, and an efficient memory model that eliminates copying memory operation when replicating the message.  \eric{need to sync with the design section}


% \eric{in this work, we takes it to an extreme by building a fault tolerance layer on top of cloud \textit{spot} instances. which it can preemptied at any time. this is challenging for latency critical tasks, creating a new instance can take up to 20 minutes (3) resiliently manage and route all the replicas across multiple cloud and regions.} 
\algname uses {Spot} Virtual Machines (VM), a cost-saving purchasing option offered by major cloud service providers\footnote{In Google Cloud Platform (GCP) and Microsoft Azure, these are called \emph{Spot Virtual Machines}. In Amazon Web Services, these are called \emph{Spot Instances}. } that are up to a 90\,\% discount off the standard on-demand pricing, because they can be \emph{terminated}\footnote{\emph{Interrupted},  \emph{terminated} and \emph{preempted} can be used interchangeably} \emph{unpredictably}. Earlier studies~\cite{10.1145/3458336.3465301} show a bioinformatics task with 24 spot virtual machines on Google Cloud Platform experiences a preemption every 36 minutes on average. 
%Re-creating and initiating a new instance with FogROS2 can take up to 20 minutes \jeff{$\leftarrow$ seems like extraneous information in this context. move elsewhere.}. 
Spot Virtual Machines (VMs) are usually used for non time-sensitive jobs that can be interrupted without significant consequences. 
With the fault tolerance layer in \algname, even time-sensitive robotics tasks can be executed on those cost-effective servers with per-request fault tolerant guarantee, enjoying the benefits of lower expenses without suffering from the drawbacks of unplanned server termination. \algname resiliently manages a pool of spot VMs across multiple cloud and regions, and recreate new spot VM if a replica gets terminated. 

% \eric{\algname achieves 2x fault tolerance with 30\% cost reduction compared to running standard cloud machines on XXX task. }
We evaluate \algname on 4 cloud robotics applications, visual object detection with YOLOv8~\cite{redmon2015you}, semantic segmentation with Segment Anything~\cite{kirillov2023segment}, motion planning with Motion Planning Templates (MPT)~\cite{ichnowski2019mpt}, and a physical Pick-and-Place task with a UR10e. We show that \algname is able to reduce deployment cost of X times, X times compared to standard non-fault-tolerant environment, and x times, X times, X times compared to standard fault-tolerant (again somewhere here emphasize that reduce long tail, won't really notice the benefit of FT on a fast run, but will notice it on a slow run)


This paper makes four contributions: (1) An open-source fault tolerant extension to FogROS2 that enables robots to leverage replicated cloud resources and stay available as long as one of the replica and network is available (2) Cost-effective and reliable Cloud Robotics deployment on spot VMs (3) Cost, fault tolerance and latency data from an experimental evaluation of \algname on 4 cloud robotics applications (4) Physical fault tolerance and cost evaluation with pick-and-place demonstration.

==> chapters_ft/introduction_v1.tex <==
% \eric{intro+related work 2 pages, design 2 pages, eval 2 pages, conclusion+references 2 pages}
% \eric{alternative names: 
% FogROS2-SPOT: Server-based Parallel Operations for fault Tolerance; 
% FogROS2-CRAFT: Cloud Robotics With Cost-Reduced And Fault-Tolerant Replicated Servers; 
% CARE - Cloud fAult-tolerant Replicated sErvers; or just FogROS2-FT }
\section{Introduction}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/use_case.png}
    \caption{\textbf{\algname Overview.} \textbf{(Top)} Cloud robotics applications, such as grasp planning, when deployed on a single cloud server become a single point of failure.
    \textbf{(Bottom)} Instead, \algname provides a cost-efficient and fault-tolerant solution that deploys unmodified ROS2 applications to multiple low-cost cloud servers, making cloud-robotics applications resilient to individual server termination and network slowdowns.
    %Without any ROS2 application modifications, \algname is more cost-efficient than conventional cloud servers launched with FogROS2, and is fault tolerant to individual server termination or slowdown.
    }
    \label{fig:intro:use_case}
\end{figure}

The complexity of foundational models~\cite{wang2021nerf,kirillov2023segment,Rashid24lifelonglerf} and sophisticated robot algorithms~\cite{ichnowski2020fog,tanwani2019fog} exceed most onboard robot computing capabilities.
% Modern robot algorithms, such as sophisticated algorithms, such as \eric{}, thing but are computationally demanding and cannot run on old or power-constrained hardware. 
Cloud robotics provides shared access to on-demand resources and services with boosted performance and simplified management, enabling the deployment of compute-intensive algorithms on low-cost, mobile robots without powerful on-board hardware, such as GPU, TPU, and high-performance CPU.
In previous research, we developed FogROS2, which enables unmodified robotics code in Robot Operating System 2 (ROS2) to offload heavy computing modules to
an independent set of % - KG
cloud hardware resources and accelerators.
FogROS2 used \emph{on-demand} servers that guarantee dedicated computing resources with high uptime (e.g., 99.99\,\%~\cite{aws_sla}). However, the network quality of service (QoS) between robots and the cloud can vary, and during rare cloud outages, robots lose all cloud-computing benefits.
Additionally, as on-demand instances can be expensive, many cloud providers offer \emph{spot VMs}\footnote{In Google Cloud Platform (GCP) and Microsoft Azure, these are called \emph{Spot Virtual Machines}. In Amazon Web Services, these are called \emph{Spot Instances}. More generally, they are also known as \emph{preemptible} or \emph{transient} machines.}  
% \jeff{TODO: define and reuse `instance', `server', or `VM' consistently. Let's avoid synonyms on this term.} \eric{skypilot paper uses spot VM. lets use VM?}
at a significantly reduced price with the caveat that they can shut down unpredictably---making them (without fault tolerance) unsuitable for many robotics applications.
In this work, we introduce \algname, a fault-tolerant extension to FogROS2~\cite{ichnowski2022fogros} 
% that is more cost-efficient than previous systems while simultaneously having 
that provides robust performance against variable network QoS, infrastructure unavailability, and stochasticity of the robotic algorithms,
% moved this next sentence from other paragraph - trinity
increasing the reliability and responsiveness of cloud robotics. % are not suitable for long duration operations. 
By adding redundancy to cloud computation, we enable cloud-robotics tasks to continue operating effectively despite the following failures: 
% \eric{However, cloud introduces factor of unreliablitiy. Traditionally when a robot's compute is broken, but regional network congestions and downtime may affect all the robots, thus affecting the entire operation. The breakdown of the computational service leads to as little as latency disturbances to safety-critical. }
 
% However, the shift towards cloud computing raises issues for the reliability of long-running, safety-critical tasks. In traditional setups, a failure in a single robot's computing resources has limited, localized effects. In contrast, cloud computing introduces vulnerabilities not present in onboard computing systems, such as regional network congestion and server outages, which can impact the operations of an entire fleet of robots. This vulnerability may lead to misconceptions that  cloud robotics are not suitable for safety-critical and long-duration operations.


% \eric{Fault tolerance becomes a requirement for cloud robotics to ensure the reliable task of every request.  however, there are a few factors that makes this challenging. (1) costly by replication, (2) hard to deploy, require engineering}
% \eric{Fault tolerance allows cloud-robotics tasks to continue operating effectively despite failures in cloud or network components, ensuring the necessary reliability for processing every request.}\eric{closing the SLA gap betweeen 0.99 and 0.9999 might make our problem too narrow. I find it hard to argue the 0.01\% downtime is a big thing. }

\begin{enumerate}[label=(\Alph*),itemindent=3em,leftmargin=0pt]
\item \textit{Resource Unavailability}: Although cloud services have high uptime and are managed by dedicated experts, outages can still occur.
For example, an AWS outage affected the availability of the iRobot  applications~\cite{irobotaws}.  In addition, spot VMs may shut down unpredictably. 
% \trinity{should these details on spot instances stay here or be moved to Related Work?}\eric{save that to related work. here we just say things can go wrong; leave the price reduction to later, here we only need "end predictably" }
% \jeff{I suggest that we should shift the focus (and introduce the robotics audience to) the notion of uptime/downtime ratios and even perhaps SLAs (e.g., \url{https://aws.amazon.com/compute/sla/}).} 

\item \textit{Resource Oversubscription}: The cloud enables flexible usage of computational resources.
For example, one can oversubscribe a system by allocating fewer resources than the sum of resources required by all robots, based on the expectation that robots will rarely all use the resources simultaneously.
Oversubscribing can improve resource utilization, but if too many robots contend for resources at once, all robots will experience performance degradation or failures.


\item \textit{Stochastic Algorithmic Latency}: Many robotic algorithms demonstrate stochastic timing behavior, such as asymptotically-optimal rapidly-exploring random tree in motion planning~\cite{ichnowski2019mpt} that relies on random sampling. Large or foundational models are also affected by the stochasticity of the operating system scheduling and buffers~\cite{li2023mathrm, li2023rt}. 
% o Performing 
% \eric{Can we make a point that the cloud can do even more than traditional onboard computing?} \ken{we already did at top of intro}
\end{enumerate}

Fault tolerance typically demands an in-depth understanding of the algorithm and specific adaptations against faults, and it involves complex deployment and management processes that require extensive engineering expertise. 
% Thus, there can be a misconception that cloud robotics are not suitable for long duration operations. However, cloud computing can provide redundancy and thus can be more reliable. % move to second paragraph of intro - goldberg
%In this work, we recognize the fact that a failure in non-cloud robot systems is fatal; in contrast, 
% However, cloud computing can provide redundancy and thus can be more reliable. 
% even though cloud networks are more prone to \jeff{Let's avoid using `prone to', we don't want to give the reader the impression that the cloud is worse than it is---that might leave them with the impression that they should avoid the cloud.} 
% regional network congestion and server outages \jeff{Let's see if we can find historical data on actual outages/uptime rates.}. 
\algname provides fault tolerance for heterogeneous stateless robotic algorithms without requiring ROS2 application modifications. It simultaneously dispatches requests to identical services deployed in multiple cloud data centers and uses the first response received from the replicated services. This model significantly increases the probability of getting timely responses as long as at least one replica and network remains operational and responsive. %\jeff{`timely` sounds like its overpromsing too. e.g., all services are slow means it will be slow (but still faster than the slowest). Is there another wording?} \eric{}
We design a replication-aware routing network that allows resilient and location independent connectivity that persists even if the service is restarted on a different machine. 



% \eric{specifically use replication to for fault tolerance, which further leads to following challenges: (1) ROS2 programming model does not consider replication (2) replicating and dispatching requests across replicas become computationally expensive, }
 

%We propose a compute-efficient threading model for asynchronously processing the requests, and an efficient memory model that eliminates copying memory operation when replicating the message.  \eric{need to sync with the design section}


% \eric{in this work, we takes it to an extreme by building a fault tolerance layer on top of cloud \textit{spot} instances. which it can preemptied at any time. this is challenging for latency critical tasks, creating a new instance can take up to 20 minutes (3) resiliently manage and route all the replicas across multiple cloud and regions.} 

%Re-creating and initiating a new instance with FogROS2 can take up to 20 minutes \jeff{$\leftarrow$ seems like extraneous information in this context. move elsewhere.}. 
To reduce the cost of launching
independent % -KG
replicated services, \algname 
can deploy to spot VMs. %, which are usually used for non time-sensitive jobs that can be interrupted without significant consequences. <- interesting, but not particularly relevant to target audience -JI
With \algname, even time-sensitive robotics tasks can be executed on those cost-effective servers with per-request fault tolerant characteristics, enjoying the benefits of lower expenses without suffering from the drawbacks of unplanned server shutdown. \algname resiliently manages a pool of spot VMs across multiple cloud and regions, and recreates a new spot VM whenever a replica gets terminated. 

% \eric{\algname achieves 2x fault tolerance with 30\% cost reduction compared to running standard cloud machines on XXX task. }
We evaluate \algname on 4 cloud-robotics applications: object detection with YOLOv8~\cite{redmon2015you}, semantic segmentation with Segment Anything (SAM)~\cite{kirillov2023segment}, motion planning with Motion Planning Templates (MPT)~\cite{ichnowski2019mpt}, and a physical pick-and-place task with a UR10e. In experiments,
\algname reduces latency by up to 1.16x in motion planning, including a 5.53x reduction on 99 Percentile (P99), a metric for long-tail latency faults; and \algname reduces average inference latency by 2.1x and P99 latency of object detection by 3.9x under network slowdown. \algname improves SAM's P99 latency by 1.96x when compute resources is contended. 
%We show that \algname is able to reduce deployment cost of X times, X times compared to standard non-fault-tolerant environment, and x times, X times, X times compared to standard fault-tolerant. \trinity{TODO: numbers}


This paper makes four contributions: (1) an open-source fault-tolerant extension to FogROS2 that enables robots to use replicated, independent cloud resources across different clouds for capacity and availability and stay available as long as one of the replicas and subnetworks is available; (2) cost-effective deployment using spot VMs; (3) cost, fault tolerance, and latency data from an experimental evaluation of \algname on 3 simulated cloud robotics applications; (4) experimental evaluation with a physical robot performing a scan-pick-and-place task.

==> chapters_ft/related_work.tex <==
\section{Related Work}

% \eric{skeleton: three paragraphs (1) cloud robotics, (2) latency (vpn(fogros2), fogros-LS paper, sgc) (3) Cloud pricing: Sky, spot instance papers, fogros sky} 
% \trinity{second draft - 03/05 2:45pm}

% 1. cloud robotics
\paragraph*{Cloud and Fog Robotics}
The use of cloud computing resources for robots, conceptualized as cloud robotics~\cite{kehoe2015survey}, has become increasingly relevant
as large models (e.g., NeRF~\cite{wang2021nerf}, SAM~\cite{kirillov2023segment} and LERF~\cite{Rashid24lifelonglerf} for visual perception) and other computationally demanding algorithms (e.g., MPPI for path planning) are integrated in robotic applications.
Following the Fog Computing paradigm~\cite{bonomi2012fog}, Fog Robotics~\cite{gudi2017fog} utilizes edge resources to improve performance, enabling the viability cloud computing for a multitude of robotics applications, including grasp planning~\cite{tanwani2019fog}, motion planning~\cite{ichnowski2020fog}, visual servoing~\cite{tian2019fog}, and human-robot interaction~\cite{gudi2018fog}.
In the FogROS2 series of work, we address several concerns of using cloud compute for robotics.
FogROS2~\cite{chen2021fogros} is a cloud robotics framework officially supported by ROS2~\cite{macenski2022robot}.
%In terms of network architecture, 
FogROS2 focused on optimizing for a single cloud and robot using a Virtual Private Network (VPN). Extensions of this work has addressed
% multi-robot and multi-cloud capabilities.
the questions of connectivity, latency, and cost.
\sgc (Secure and Global Connectivity)~\cite{chen2023sgc} enables secure communication between distributed ROS2 robot nodes.
% Additionally, we address latency concerns in


% 2. latency, fogros-ls, sgc
\paragraph*{Multi-Cloud Robotics}
FogROS2 is the first multi-cloud robotics that offloads robotics applications to multiple cloud service providers. 
FogROS2-Config~\cite{chen2024fogrosconfig} extend FogROS2 to  navigate available cloud machine selection that meets user-specified time and cost per request.
\algname uses multi-cloud Spot VMs to reduce the cost of the deployment. Spot VMs 
are one such cost-saving purchasing option offered by major cloud service providers that are up to a 90\,\% discount off the standard on-demand pricing, because they can be \emph{preempted}\footnote{\emph{Preempted},  \emph{shut down} and \emph{interrupted} are used interchangeably.} \emph{unpredictably}~\cite{amazon2021spot}. This creates trade-off between the reduced price of spot VMs and having to build an infrastructure handling shutdowns and restarts~\cite{li2016spotpricereview}.
The rates of preemption are highly variable across regions and instance types, from 3\,\% to over 20\,\% chance of preemption per day.
Spot VM prices are also variable, and can fluctuate over the course of a day.
Extensive research has been done to predict spot pricing using statistical models~\cite{javadi2011spotpricemodeling,singh2015spotpricepredict} and learning methods~\cite{baughman2018spotpricelstm,khandelwal2020spotpricerrf}.
Due to their unreliable nature, spot VMs were not considered as part of the machine selection in FogROS2 and FogROS2-Config.

% FogROS2-Config focuses on selecting a cloud machine with the ideal hardware specifications, but cloud providers offer a wide variety of pricing options that differ beyond hardware.
% Cloud providers offer a wide variety of pricing options \cite{wu2019cloudpricing} based on hardware specifications and availability.



% \cite{lee2023spoteconomics} \cite{george2019awsspot}.

\paragraph*{Fault Tolerance for Latency Sensitive Applications} 
% A fault tolerant system is naturally compatible with spot VMs. 
A fault tolerant system is typically based on  \emph{failover}, dynamically switching to one of the machines upon failure of one machine, and \emph{redundancy} by duplicated machines ensuring operation in case of a failure on one system.
%\trinity{maybe clarify a fault tolerant system implement one or more of these strategies.}
FogROS2-LS (Latency Sensitive)~\cite{chen2024fogrosls} implements failover strategy by enabling robots to flexibly connect with one of many servers, but the system takes time to discover and recover from faults by switching to another server that meets latency requirements. 
~\citet{lee2017deepspotcloud} enables fault tolerance on spot VMs for deep learning by actively checkpointing and recovering from the failure. 
On redundancy, \citet{schafhalter2023cloudav} improves the responsiveness of autonomous vehicles by performing operations on both vehicle and cloud. 
On fault tolerance of spot VMs, 
\citet{voorsluys2012reliablespot,poola2016spot,pergentino2019mults} demonstrate spot instances can be used as a cost-efficient setup. However, they focus on the cost optimization on a single server. \citet{alieldin2019spotweb} uses redundancy of spot VMs on web services. Fault tolerance of continuous and latency-sensitive robotic operations is understudied. With \algname, off-the-shelf robotics applications can run in fault-tolerant environment without the awareness of the robotic application developers.



% \eric{merge fogros2(sky) with spot instances; include related work for fault tolerance}

% \textbf{Fault Tolerance}
% ... \citet{hasan2018ftsurvey} \trinity{there are different ``levels" of fault tolerance; proactive vs reactive measures, etc. should we go into this?}
% \eric{a high level overview of existing methods is fine. We say: we leverage the uniqueness of the cloud (if there is no existing work on that).}


\section{System Assumptions and Features}

\subsection{System Assumptions}
We assume the application can be partitioned as a \emph{robot} that sends sensor data as requests and await control instructions as response from a \emph{service} that encapsulates the algorithm.
We assume that all servers, networks, and faults are independent. 
%The robot needs to have a stable connection to at least one of the cloud machines. The application needs to computational capacity of the cloud needs to handle the request requirement to receive timely response. 
The services need to be stateless to achieve fault tolerance without application awareness, or applications needs to use well-defined interfaces from \algname to make the states consistent.
% It cannot protect from application software bugs.  % omit - goldberg
% \eric{assume each svm is independent and failures are not correlated}

We assume the application is implemented in ROS2, the de-facto platform for building robotics applications. In ROS2, the computational units (\emph{client} and \emph{service}) are abstracted into \emph{ROS2 nodes}. \algname assumes the nodes are connected by ROS2 service communication model~\cite{ros2_service}.


\subsection{Fault Tolerance Properties}

\algname achieves fault tolerance with the following properties: 

\begin{enumerate}
    \item \textbf{Zero Downtime at Faults}. \algname enables fine-grained request-level fault tolerance that ensures a requests can be fulfilled as long as at least one replica and network remains operational. 
    \item \textbf{Algorithm-Agnostic}. \algname operates independently of the specific algorithms used in applications as long as it is stateless.
    \item \textbf{Failure Cause-Agnostic}. \algname does not need to be tailored to specific failure, and remains functional as long as at least one service is available and connected.
    \item \textbf{Hardware-Agnostic}. \algname is agnostic to heterogeneous hardware resource options provided by the cloud, supporting simultaneous use of different resource types and fault tolerance level. 
    % on-demand and spot instances, and even different spec instances (e.g., low-spec on-demand for up-time, and high-spec spot for speed) 
    \item \textbf{Multi-cloud, Multi-region}. Since the failure may occur to a specific region or cloud provider, \algname, as part of the Sky Computing paradigm~\cite{chasins2022sky}~\cite{yang2023skypilot}, offers a unified interface for interacting with various cloud service providers and uses cloud computing resources across different clouds simultaneously. 
    % \item \textbf{Seamless ROS2 Application Integration:} With \algname, there's no need for modifications to existing ROS2 applications; they can be offloaded to the cloud and will function as though all ROS2 components were located on a single machine. 
\end{enumerate}



\subsection{\algname Failure Qualification}
% \ken{qualify as P(failure) = 1-P(fail1)*P(fail2)}
Multiple cloud servers can provide fault tolerance to region or server-specific compute or network failures. 
% \trinity{from Christian J: ``Maybe important to discuss: which types of failures are targeted in detail, and can we quantify the likelihood of these failures (eg SLAs)? The paper is stronger if we don't need the cost aspect to justify its usefulness"}
We assume the robot has a persistent and stable connection to at least one of the cloud servers. 
% Since \algname can launch cloud servers across different regions and cloud service providers, the probability of simultaneous failures from independent cloud service providers or regions is independent.
% REFRAME MATH SECTION
% % We qualify the failure of \algname as following:  The Spot VM can be terminated unpredictably. 
% % We define the failure as following: 
% The probability of a server failing can be estimated as:
% \[
% P(\text{Failure of VM}_i) = 1-\frac{\text{uptime of VM}_i}{\text{uptime}_i + \text{recovery time}_i}
% \]

% % \ken{VM to Spot VM} \eric{actually here we can be more general, as spot VM's failure is just a type of VM failure}
% % As a result, the failure of \algname can be qualified as 
% As a result, the probability of a system failure with N replicated VMs is:
% \[
% % P(\text{Failure}) = 1 - \prod_{i \in \Theta} P(\text{Failure of VM}_i)
% P(\text{Failure}) = 1 - \prod_{i \in N} P(\text{Failure of VM}_i)
% \]
% % where $\Theta$ is the set for all the VMs. \eric{this formulation assumes the number of replica is constant}
% NEWLY REFRAMED MATH SECTION
The probability of a VM failing at any moment in time is% \jeff{This is at any moment in time, correct? We should state that explicitly if so. If not, can we clarify?}
\[
P_{\text{VM}_i}(\text{failure}) =
% 1-\frac{\text{uptime}_{\text{VM}_i}}{\text{uptime}_{\text{VM}_i} + \text{recovery time}_{\text{VM}_i}}
\frac{\text{recovery\_time}_{\text{VM}_i}}{\text{uptime}_{\text{VM}_i} + \text{recovery\_time}_{\text{VM}_i}}, % <- punctuate equations when used in sentences
\]
and the probability of a system failure with $N$ spot VMs is
\[
P_{\text{system}}(\text{failure}) = \prod_{i \in N} P_{\text{VM}_i}(\text{failure}).
\]
% Given the desired maximum failure rate for the system $P_{\text{system}}(\text{failure}) = \epsilon$ and assuming the preemption rate for spot VMs $P_{\text{VM}_i}(\text{failure}) = \delta$, we can calculate the required $N$ number of replicas as
Given a desired maximum failure rate for the system and the failure rate for all VMs used, we can calculate the required number of VM replicas as
   \[  N = \left\lceil \frac{\log{P_{\text{VM}}(\text{failure})}}{\log{P_{\text{system}}(\text{failure})}} \right\rceil. \]

To reduce the probability of failure, one can either increase the number of replicas, or use a combination of spot and on-demand instances. 
% \jeff{The next sentences should be framed as an example. In particular, we cannot expect the preemption rate to be the same throughout the year, or for years to come.}
For example, a spot VM is preempted every 15 hours on average from experiments by Skypilot paper~\cite{yang2023skypilot} and re-creating and initiating a new instance with FogROS2 can take up to 20-minute downtime~\cite{chen2021fogros}, the probability of simultaneous preemptions with two spot VMs is less than 0.05\,\%, fulfilling the Service Level Agreement of AWS on non-spot VMs~\cite{aws_sla}. 
%\trinity{suggestion: calculate using the typically provided spot rates of preemption chance per day (from 5\% to $>$20\%). Using a 20\% machine would still result in $<$0.05\% failure}
% 15 hours is from skypilot paper 


% Probability is lowered if more replicas are used. % move to earlier - goldberg 
% One can also mix the cloud server with spot VM to further reduce the failure rate. % ?? - goldberg

\subsection{New Features}

\algname is distinguished from previous work with the following features: 
% \jeff{I'm a little concerned that this mostly reads as 1. FT, 2. other, 3. FT, 4. FT, 5. FT, 6. other, 7. other. Not sure the fix. It could be to just remove ``fault tlerance'' from a few. Or make the list hierarchical. Or just ignore this concern.} 
% \eric{@Jeff, see the updated - I moved FT before failure qualification. I think this may flow better: we guard against following faults ... and we qualify our failures as ...}
\begin{enumerate}
    \item \textbf{Cost-effectiveness}.  \algname can provide significantly lower cost by using spot VMs. 
    % \jeff{Can we add `Mixed resource type' to highlight that one can mix on-demand and spot instances, and even different spec instances (e.g., low-spec on-demand for up-time, and high-spec spot for speed)
    % } \eric{moved this to FT}
    \item \textbf{Scalability} \algname allows robots to launch a adjustable 
    % \jeff{be a bit more specific with the `scalable' number here---otherwise this is defining the Scalability feature as being scalable.}
    % \trinity{variable? adjustable?}
    number of machines to reduce the probability that all the replica service deployments are not available. 
    \item \textbf{Flexibility} \algname is flexible to the choice of available hardware resources. For example, one can mix low-specification on-demand cloud machines for up-time with high-specification spot VMs for speed. 
    \item \textbf{Adaptive and Resilient recovery} \algname automatically recovers from service interruptions, preserving the intended level of fault tolerance automatically.
    % \item \textbf{Seamless ROS2 Application Integration:} With \algname, there's no need for modifications to existing ROS2 applications; they can be offloaded to the cloud and will function as though all ROS2 components were located on a single machine. 
\end{enumerate}


==> chapters_ft/related_work_v0.tex <==
\section{Related Work}

% \eric{skeleton: three paragraphs (1) cloud robotics, (2) latency (vpn(fogros2), fogros-LS paper, sgc) (3) Cloud pricing: Sky, spot instance papers, fogros sky} 
\trinity{second draft - 03/05 2:45pm}

% 1. cloud robotics
\textbf{Cloud and Fog Robotics}.
The use of cloud computing resources for robots, conceptualized as cloud robotics \cite{kehoe2015survey}, has become increasingly relevant
as large models (e.g. NeRF \cite{wang2021nerf} and SAM \cite{kirillov2023segment} for visual perception) and other computationally demanding algorithms (e.g. MPPI for path planning) are integrated in robotic applications.
\trinity{maybe include autonomous vehicle from Prof. Stoica \citet{schafhalter2023cloudav}} \eric{yes peter's paper is definitely relevant}
Following the Fog Computing paradigm \cite{bonomi2012fog}, Fog Robotics \cite{gudi2017fog} utilizes edge resources to improve performance, enabling the viability cloud computing for a multitude of robotics applications, including grasp planning~\cite{tanwani2019fog}, motion planning~\cite{ichnowski2020fog}, visual servoing~\cite{tian2019fog}, and human-robot interaction~\cite{gudi2018fog}.
In the FogROS2 series of work, we address several concerns of using cloud compute for robotics.

% 2. latency, fogros-ls, sgc
\textbf{FogROS2 and Extensions}.
FogROS2 \cite{chen2021fogros} is a cloud robotics framework officially supported by ROS2 \cite{macenski2022robot}.
In terms of network architecture, FogROS2 focused on optimizing for a single cloud and robot using a Virtual Private Network (VPN). Extensions of this work has addressed
% multi-robot and multi-cloud capabilities.
the questions of connectivity, latency, and cost.
\sgc (Secure and Global Connectivity) \cite{chen2023fogros} connects distributed ROS2 nodes in a peer-to-peer network, enabling secure communication between robots.
% Additionally, we address latency concerns in
FogROS2-LS (Latency Sensitive) \cite{chen2024fogrosls} adopts \emph{anycast} \cite{ballani2005anycast} communication so that a robot can flexibly switch to using one of many servers to meet latency requirements.
% FogROS2-Pilot \cite{chen2024sky} is able to select a cloud machine across multiple clouds (Amazon Web Services, Google Cloud Platform, Microsoft Azure) by extending SkyPilot \cite{yang2023skypilot}, an "intercloud broker." 
% In FogROS2-Pilot \cite{chen2024sky}, we follow the philosophy of Sky Computing \cite{chasins2022sky}, where cloud compute across providers are treated as one commodity.
% By querying SkyPilot \cite{yang2023skypilot}, an intercloud broker,
% FogROS2-Pilot selects a cloud machine across multiple clouds\footnote{The supported clouds are Amazon Web Services (AWS), Google Cloud Platform (GCP), and Microsoft Azure. \trinity{are there others?}} that meets user-specified time and cost per request.
FogROS2-Pilot \cite{chen2024sky} alleviates roboticists from having to navigate hundreds of available cloud machine by automatically selecting a that meets user-specified time and cost per request.


% 3. cloud pricing, spot instance, fogros sky
\textbf{Spot VMs}.
FogROS2-Pilot focuses on selecting a cloud machine with the ideal hardware specifications, but cloud providers offer a wide variety of pricing options that differ beyond hardware.
% Cloud providers offer a wide variety of pricing options \cite{wu2019cloudpricing} based on hardware specifications and availability.
Spot VMs\footnote{In Google Cloud Platform (GCP) and Microsoft Azure, these are called \emph{Spot Virtual Machines}. In Amazon Web Services, these are called \emph{Spot Instances}. More generally, they are also known as \emph{preemptible} or \emph{transient} machines.}
are one such cost-saving purchasing option offered by major cloud service providers that are up to a 90\,\% discount off the standard on-demand pricing, because they can be \emph{preempted}\footnote{\emph{Preempted},  \emph{terminated} and \emph{interrupted} can be used interchangeably.} \emph{unpredictably} \cite{amazon2021spot}. 
The rates of preemption are highly variable across regions and instance types, from 3\% to over 20\% chance of preemption per day.
The prices are also variable, and can even fluctuate over the course of a single day.
Extensive research has been done to predict spot pricing using statistical models \cite{javadi2011spotpricemodeling} \cite{singh2015spotpricepredict} and learning methods \cite{baughman2018spotpricelstm} \cite{khandelwal2020spotpricerrf}.
Due to their unreliable nature and lack of guarantees, spot VMs were not considered as part of the machine selection in FogROS2-Pilot.
From a user perspective, there is an economic trade-off of the reduced price of spot VMs and having to build an infrastructure handling shutdowns and restarts \cite{li2016spotpricereview}.
% \cite{lee2023spoteconomics} \cite{george2019awsspot}.

Fortunately, a fault tolerant system is naturally compatible with spot VMs. The core components of a fault tolerant system are \emph{redundancy}, duplicated machines ensuring operation in case of a failure on one system, and \emph{failover}, dynamically switching to one of the replica machines upon failure of one machine.
\citet{voorsluys2012reliablespot}, \citet{poola2016spot}, and \citet{pergentino2019mults} among others have demonstrated that spot instances can be used as a cost-efficient, fault-tolerant setup.
Spot instances have been used successfully for multiple applications including web services \cite{alieldin2019spotweb}, deep learning \cite{lee2017deepspotcloud}, but spot usage has not yet been explored for robotics.

\eric{merge fogros2(sky) with spot instances; include related work for fault tolerance}

% \textbf{Fault Tolerance}
% ... \citet{hasan2018ftsurvey} \trinity{there are different ``levels" of fault tolerance; proactive vs reactive measures, etc. should we go into this?}
% \eric{a high level overview of existing methods is fine. We say: we leverage the uniqueness of the cloud (if there is no existing work on that).}


\section{System Assumptions and Features}

\subsection{System Assumptions}
In this work, we assume the applications adhere to ROS2 request-response communication model. The application can be partitioned as a client that sends sensor data as requests and await control instructions as response, and service implemented as ROS2 services that can be offloaded to the cloud. 
%The robot needs to have a stable connection to at least one of the cloud machines. The application needs to computational capacity of the cloud needs to handle the request requirement to receive timely response. 
The services need to be stateless to achieve fault tolerance without application awareness, or applications needs to use well-defined interfaces from \algname to make the states consistent.
% It cannot protect from application software bugs.  % omit - goldberg
% \eric{assume each svm is independent and failures are not correlated}

\subsection{\algname Failure Qualification}
% \ken{qualify as P(failure) = 1-P(fail1)*P(fail2)}
Multiple cloud servers can provide fault tolerance independent against region or server-specific compute or network failures. 
% \trinity{from Christian J: ``Maybe important to discuss: which types of failures are targeted in detail, and can we quantify the likelihood of these failures (eg SLAs)? The paper is stronger if we don't need the cost aspect to justify its usefulness"}
We assume the robot has a persistent and stable connection to at least one of the cloud servers. 
Since \algname can launch cloud servers across different regions and cloud service providers, the probability of simultaneous failures from independent cloud service providers or regions is independent.

% REFRAME MATH SECTION
% % We qualify the failure of \algname as following:  The Spot VM can be terminated unpredictably. 
% % We define the failure as following: 
% The probability of a server failing can be estimated as:
% \[
% P(\text{Failure of VM}_i) = 1-\frac{\text{uptime of VM}_i}{\text{uptime}_i + \text{recovery time}_i}
% \]

% % \ken{VM to Spot VM} \eric{actually here we can be more general, as spot VM's failure is just a type of VM failure}
% % As a result, the failure of \algname can be qualified as 
% As a result, the probability of a system failure with N replicated VMs is:
% \[
% % P(\text{Failure}) = 1 - \prod_{i \in \Theta} P(\text{Failure of VM}_i)
% P(\text{Failure}) = 1 - \prod_{i \in N} P(\text{Failure of VM}_i)
% \]
% % where $\Theta$ is the set for all the VMs. \eric{this formulation assumes the number of replica is constant}
% NEWLY REFRAMED MATH SECTION
The probability of one VM failing can be estimated as
\[
P_{\text{VM}_i}(\text{failure}) = 1-\frac{\text{uptime}_{\text{VM}_i}}{\text{uptime}_{\text{VM}_i} + \text{recovery time}_{\text{VM}_i}}
\]
and the probability of a system failure with $N$ replicas is
\[
P_{\text{system}}(\text{failure}) = \prod_{i \in N} P_{\text{VM}_i}(\text{failure})
\]
% Given the desired maximum failure rate for the system $P_{\text{system}}(\text{failure}) = \epsilon$ and assuming the preemption rate for spot VMs $P_{\text{VM}_i}(\text{failure}) = \delta$, we can calculate the required $N$ number of replicas as
Given the desired maximum failure rate for the system and estimating the failure rate for all VMs used, we can calculate the required $N$ number of VM replicas as
   \[  N = \left\lceil \frac{\log{P_{\text{VM}}(\text{failure})}}{\log{P_{\text{system}}(\text{failure})}} \right\rceil \]

To reduce the probability of failure, one can either increase the number of replicas, or use a combination of spot and on-demand instances. 
Assuming a spot VM is preempted every 15 hours on average and re-creating and initiating a new instance with FogROS2 can take up to 20-minute downtime, the probability of simultaneous preemptions with two spot VMs is less than 0.05\%. \trinity{suggestion: calculate using the typically provided spot rates of preemption chance per day (from 5\% to $>$20\%). Using a 20\% machine would still result in $<$0.05\% failure}
% Probability is lowered if more replicas are used. % move to earlier - goldberg 
% One can also mix the cloud server with spot VM to further reduce the failure rate. % ?? - goldberg

\subsection{New Features}

\algname is distinguished from previous work with the following features: 

\begin{enumerate}
    \item \textbf{Fault Tolerance}. \algname features \textit{per-request} fault tolerance, ensuring requests can be fulfilled as long as at least one replica and network remains operational.
    \item \textbf{Cost-Effectiveness}.  \algname can provide significantly lower cost by using spot VMs
    \item \textbf{Algorithm Agnostic Fault Tolerance}. \algname operates independently of the specific algorithms used in applications as long as it is stateless 
    \item \textbf{Failure Cause Agnostic}. \algname does not need to be tailored to specific failure scenarios, and remains functional as long as at least one service is available and connected.
    \item \textbf{Multi-Cloud, Multi-Region Fault Tolerance}. Since the failure may occur to a specific region or cloud provider, \algname, as part of the Sky Computing paradigm, offers a unified interface for interacting with various cloud service providers and leverages cloud computing resources across different clouds simultaneously. 
    \item \textbf{Scalability}. \algname allows robots to launch a scalable number of machines to set the probability that all the replica service deployments are not available. 
    \item \textbf{Adaptive and Resilient Recovery}. \algname automatically recovers from service interruptions, preserving the intended level of fault tolerance automatically.
    % \item \textbf{Seamless ROS2 Application Integration:} With \algname, there's no need for modifications to existing ROS2 applications; they can be offloaded to the cloud and will function as though all ROS2 components were located on a single machine. 
\end{enumerate}

==> chapters_ft/related_work_v1.tex <==
\section{Related Work}

% \eric{skeleton: three paragraphs (1) cloud robotics, (2) latency (vpn(fogros2), fogros-LS paper, sgc) (3) Cloud pricing: Sky, spot instance papers, fogros sky} 
% \trinity{second draft - 03/05 2:45pm}

% 1. cloud robotics
\paragraph*{Cloud and Fog Robotics}
The use of cloud computing resources for robots, conceptualized as cloud robotics~\cite{kehoe2015survey}, has become increasingly relevant
as large models (e.g., NeRF~\cite{wang2021nerf}, SAM~\cite{kirillov2023segment} and LERF~\cite{Rashid24lifelonglerf} for visual perception) and other computationally demanding algorithms (e.g., MPPI for path planning) are integrated in robotic applications.
Following the Fog Computing paradigm~\cite{bonomi2012fog}, Fog Robotics~\cite{gudi2017fog} utilizes edge resources to improve performance, enabling the viability cloud computing for a multitude of robotics applications, including grasp planning~\cite{tanwani2019fog}, motion planning~\cite{ichnowski2020fog}, visual servoing~\cite{tian2019fog}, and human-robot interaction~\cite{gudi2018fog}.
In the FogROS2 series of work, we address several concerns of using cloud compute for robotics.
FogROS2~\cite{chen2021fogros} is a cloud robotics framework officially supported by ROS2~\cite{macenski2022robot}.
%In terms of network architecture, 
FogROS2 focused on optimizing for a single cloud and robot using a Virtual Private Network (VPN). Extensions of this work has addressed
% multi-robot and multi-cloud capabilities.
the questions of connectivity, latency, and cost.
\sgc (Secure and Global Connectivity)~\cite{chen2023sgc} enables secure communication between distributed ROS2 robot nodes.
% Additionally, we address latency concerns in


% 2. latency, fogros-ls, sgc
\paragraph*{Multi-Cloud Robotics}
FogROS2 is the first multi-cloud robotics that offloads robotics applications to multiple cloud service providers. 
FogROS2-Config~\cite{chen2024fogrosconfig} extend FogROS2 to  navigate available cloud machine selection that meets user-specified time and cost per request.
\algname uses multi-cloud Spot VMs to reduce the cost of the deployment. Spot VMs 
are one such cost-saving purchasing option offered by major cloud service providers that are up to a 90\,\% discount off the standard on-demand pricing, because they can be \emph{preempted}\footnote{\emph{Preempted},  \emph{shut down} and \emph{interrupted} are used interchangeably.} \emph{unpredictably}~\cite{amazon2021spot}. This creates trade-off between the reduced price of spot VMs and having to build an infrastructure handling shutdowns and restarts~\cite{li2016spotpricereview}.
The rates of preemption are highly variable across regions and instance types, from 3\,\% to over 20\,\% chance of preemption per day.
Spot VM prices are also variable, and can fluctuate over the course of a day.
Extensive research has been done to predict spot pricing using statistical models~\cite{javadi2011spotpricemodeling,singh2015spotpricepredict} and learning methods~\cite{baughman2018spotpricelstm,khandelwal2020spotpricerrf}.
Due to their unreliable nature, spot VMs were not considered as part of the machine selection in FogROS2 and FogROS2-Config.

% FogROS2-Config focuses on selecting a cloud machine with the ideal hardware specifications, but cloud providers offer a wide variety of pricing options that differ beyond hardware.
% Cloud providers offer a wide variety of pricing options \cite{wu2019cloudpricing} based on hardware specifications and availability.



% \cite{lee2023spoteconomics} \cite{george2019awsspot}.

\paragraph*{Fault Tolerance for Latency Sensitive Applications} 
% A fault tolerant system is naturally compatible with spot VMs. 
A fault tolerant system is typically based on \emph{redundancy} by duplicated machines ensuring operation in case of a failure on one system, and \emph{failover}, dynamically switching to one of the machines upon failure of one machine.
FogROS2-LS (Latency Sensitive)~\cite{chen2024fogrosls} adopts \emph{anycast}~\cite{ballani2005anycast} communication so that a robot can flexibly connect to using one of many servers, but the system takes time to discover and recover from faults by switching to another server that meets latency requirements.
\citet{schafhalter2023cloudav} improves the responsiveness of autonomous vehicles by performing operations on both vehicle and cloud. 
\citet{wu2018visual} statistically models and detects anomalous time series events.
\citet{voorsluys2012reliablespot,poola2016spot,pergentino2019mults} demonstrate spot instances can be used as a cost-efficient, fault-tolerant setup. However, they focus on the cost optimization on a single operation, while the design of reducing faults of continuous and latency-sensitive robotic operations is understudied. Prior work also designed  applications to fault tolerance environment with spot VMs, such as web services~\cite{alieldin2019spotweb} and deep learning~\cite{lee2017deepspotcloud}. \algname can automatically offload off-the-shelf robotics applications to fault-tolerant multi-cloud environment without the awareness of the robotic application developers.



% \eric{merge fogros2(sky) with spot instances; include related work for fault tolerance}

% \textbf{Fault Tolerance}
% ... \citet{hasan2018ftsurvey} \trinity{there are different ``levels" of fault tolerance; proactive vs reactive measures, etc. should we go into this?}
% \eric{a high level overview of existing methods is fine. We say: we leverage the uniqueness of the cloud (if there is no existing work on that).}


\section{System Assumptions and Features}

\subsection{System Assumptions}
We assume
that all servers, networks, and faults are independent, and that 
% \trinity{added this from Goldberg's notes, maybe reformat/reword this}
the applications adhere to ROS2 service communication model. The application can be partitioned as a client that sends sensor data as requests and await control instructions as response, and service implemented as ROS2 services that can be offloaded to the cloud. 
%The robot needs to have a stable connection to at least one of the cloud machines. The application needs to computational capacity of the cloud needs to handle the request requirement to receive timely response. 
The services need to be stateless to achieve fault tolerance without application awareness, or applications needs to use well-defined interfaces from \algname to make the states consistent.
% It cannot protect from application software bugs.  % omit - goldberg
% \eric{assume each svm is independent and failures are not correlated}

\subsection{\algname Failure Qualification}
% \ken{qualify as P(failure) = 1-P(fail1)*P(fail2)}
Multiple cloud servers can provide fault tolerance to region or server-specific compute or network failures. 
% \trinity{from Christian J: ``Maybe important to discuss: which types of failures are targeted in detail, and can we quantify the likelihood of these failures (eg SLAs)? The paper is stronger if we don't need the cost aspect to justify its usefulness"}
We assume the robot has a persistent and stable connection to at least one of the cloud servers. 
% Since \algname can launch cloud servers across different regions and cloud service providers, the probability of simultaneous failures from independent cloud service providers or regions is independent.
% REFRAME MATH SECTION
% % We qualify the failure of \algname as following:  The Spot VM can be terminated unpredictably. 
% % We define the failure as following: 
% The probability of a server failing can be estimated as:
% \[
% P(\text{Failure of VM}_i) = 1-\frac{\text{uptime of VM}_i}{\text{uptime}_i + \text{recovery time}_i}
% \]

% % \ken{VM to Spot VM} \eric{actually here we can be more general, as spot VM's failure is just a type of VM failure}
% % As a result, the failure of \algname can be qualified as 
% As a result, the probability of a system failure with N replicated VMs is:
% \[
% % P(\text{Failure}) = 1 - \prod_{i \in \Theta} P(\text{Failure of VM}_i)
% P(\text{Failure}) = 1 - \prod_{i \in N} P(\text{Failure of VM}_i)
% \]
% % where $\Theta$ is the set for all the VMs. \eric{this formulation assumes the number of replica is constant}
% NEWLY REFRAMED MATH SECTION
The probability of a VM failing at any moment in time is% \jeff{This is at any moment in time, correct? We should state that explicitly if so. If not, can we clarify?}
\[
P_{\text{VM}_i}(\text{failure}) =
% 1-\frac{\text{uptime}_{\text{VM}_i}}{\text{uptime}_{\text{VM}_i} + \text{recovery time}_{\text{VM}_i}}
\frac{\text{recovery\_time}_{\text{VM}_i}}{\text{uptime}_{\text{VM}_i} + \text{recovery\_time}_{\text{VM}_i}}, % <- punctuate equations when used in sentences
\]
and the probability of a system failure with $N$ spot VMs is
\[
P_{\text{system}}(\text{failure}) = \prod_{i \in N} P_{\text{VM}_i}(\text{failure}).
\]
% Given the desired maximum failure rate for the system $P_{\text{system}}(\text{failure}) = \epsilon$ and assuming the preemption rate for spot VMs $P_{\text{VM}_i}(\text{failure}) = \delta$, we can calculate the required $N$ number of replicas as
Given a desired maximum failure rate for the system and the failure rate for all VMs used, we can calculate the required number of VM replicas as
   \[  N = \left\lceil \frac{\log{P_{\text{VM}}(\text{failure})}}{\log{P_{\text{system}}(\text{failure})}} \right\rceil. \]

To reduce the probability of failure, one can either increase the number of replicas, or use a combination of spot and on-demand instances. 
\jeff{The next sentences should be framed as an example. In particular, we cannot expect the preemption rate to be the same throughout the year, or for years to come.}
A spot VM is preempted every 15 hours on average~\cite{yang2023skypilot} and re-creating and initiating a new instance with FogROS2 can take up to 20-minute downtime~\cite{chen2021fogros}, the probability of simultaneous preemptions with two spot VMs is less than 0.05\,\%. 
%\trinity{suggestion: calculate using the typically provided spot rates of preemption chance per day (from 5\% to $>$20\%). Using a 20\% machine would still result in $<$0.05\% failure}
% 15 hours is from skypilot paper 


% Probability is lowered if more replicas are used. % move to earlier - goldberg 
% One can also mix the cloud server with spot VM to further reduce the failure rate. % ?? - goldberg

\subsection{New Features}

\algname is distinguished from previous work with the following features: \jeff{I'm a little concerned that this mostly reads as 1. FT, 2. other, 3. FT, 4. FT, 5. FT, 6. other, 7. other. Not sure the fix. It could be to just remove ``fault tlerance'' from a few. Or make the list hierarchical. Or just ignore this concern.}

\begin{enumerate}
    \item \textbf{Fault tolerance}. \algname features \textit{per-request} fault tolerance, ensuring requests can be fulfilled as long as at least one replica and network remains operational.
    \item \textbf{Cost-effectiveness}.  \algname can provide significantly lower cost by using spot VMs. \jeff{Can we add `Mixed resource type' to highlight that one can mix on-demand and spot instances, and even different spec instances (e.g., low-spec on-demand for up-time, and high-spec spot for speed)}
    \item \textbf{Algorithm-agnostic fault tolerance}. \algname operates independently of the specific algorithms used in applications as long as it is stateless.
    \item \textbf{Failure cause agnostic}. \algname does not need to be tailored to specific failure, and remains functional as long as at least one service is available and connected.
    \item \textbf{Multi-cloud, multi-region fault tolerance}. Since the failure may occur to a specific region or cloud provider, \algname, as part of the Sky Computing paradigm \jeff{cite?}, offers a unified interface for interacting with various cloud service providers and leverages cloud computing resources across different clouds simultaneously. 
    \item \textbf{Scalability} \algname allows robots to launch a scalable \jeff{be a bit more specific with the `scalable' number here---otherwise this is defining the Scalability feature as being scalable.} number of machines to set the probability that all the replica service deployments are not available. 
    \item \textbf{Adaptive and resilient recovery} \algname automatically recovers from service interruptions, preserving the intended level of fault tolerance automatically.
    % \item \textbf{Seamless ROS2 Application Integration:} With \algname, there's no need for modifications to existing ROS2 applications; they can be offloaded to the cloud and will function as though all ROS2 components were located on a single machine. 
\end{enumerate}


==> tables/cost.tex <==


\begin{table}[t]
    \centering
    \footnotesize
    \scalebox{0.9}{% Scale the table to 90% of its original size
    \begin{tabular}{lcccccc}
    \toprule
            & Server & Single Server & \multicolumn{3}{c}{\algname (USD per Hour)}\\
    Application & Core &  (USD per Hour) & On-Demand & & {Spot VM} \\
    \midrule
    YOLO & 16 & 0.40 (1.17x) & 0.80 (2.34x) & & {0.34 (1x)} \\
    SAM & 4$^*$ & 0.53 (1.21x) & 1.06 (2.42x) & & {0.44 (1x)} \\
    MPT-Home & 32 & 1.79 (1.05x) & 3.58 (2.10x) & & {1.69 (1x)} \\
    MPT-Cubicles & 32 & 1.79 (1.05x) & 3.58 (2.10x) & & {1.69 (1x)} \\
    MPT-TwistyCool & 64 & 3.58 (2.13x) & 7.16 (4.26x) & & {1.68 (1x)} \\
    Pick-Scan-Place & 16 & 0.40 (1.17x) & 0.80 (2.34x) & & {0.34 (1x)} \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{\algname hourly cost (USD per Hour) comparison to a Single-Server (one on-demand cloud machine)} \algname can use two on-demand machines deployment or spot VMs. In SAM, we use Nvidia T4 GPU accelerator for the inference. \algname is cheaper to run 2 spot VMs as opposed to a single server deployment up to 2.13x. }
    \label{tab:eval:cost}
\end{table}

% \begin{table}[t]
%     \centering
%     \footnotesize
%     \begin{tabular}
%         {@{}l | @{\quad}c@{\quad} | c@{\quad}  | c@{\;} c@{\quad}c@{\;}c@{\;}c@{}}\toprule
%                     & Server &Single &  \multicolumn{3}{c}\algname  \\
%          Application & Core      &Server &   On-Demand  & & {Spot VM} \\ \midrule
%          YOLO & 16  & 0.40 (1.17x) &    0.80 (2.34x)     & & {0.34 (1x)}   \\ % spot 0.17
%          SAM & 4$^*$  & 0.53 (1.21x) &    1.06 (2.42x)    & & {0.44 (1x)} \\ % spot 0.223
%          % MPT-Apartment & 16   &0.90 (1.09x)  &  1.80 (2.18x)  &{0.82 (1x)} &  \\ % spot 0.17
%          MPT-Home        & 32   &1.79 (1.05x) & 3.58 (2.10x)  & &{1.69 (1x)} \\ 
%          MPT-Cubicles & 32  &1.79 (1.05x) &   3.58 (2.10x)    & &{1.69 (1x) }  \\ 
%          MPT-TwistyCool & 64 &3.58 (2.13x) &  7.16 (4.26x)  & &{1.68 (1x)}  \\ 
%         Pick-Scan-Place & 16  & 0.40 (1.17x) &    0.80 (2.34x)     & & {0.34 (1x)}    \\ 
%          \bottomrule
%     \end{tabular}
%     \caption{\textbf{\algname hourly cost (USD per Hour) comparison to a Single-Server (one on-demand cloud machine)}  \algname can use two on-demand machines deployment or spot VMs. In SAM, we use Nvidia T4 GPU accelerator for the inference. \algname is cheaper to run 2 spot VMs as opposed to a single server deployment up to 2.13x. \jeff{unclear, is this table showing USD/hour?  If so, label it in the column headers.} \jeff{Switch to booktabs, see latex comment for URL} } % https://nhigham.com/2019/11/19/better-latex-tables-with-booktabs/
%     \label{tab:eval:cost}
% \end{table}


% % \begin{table}[t]
% %     \centering
% %     \footnotesize
% %     \begin{tabular}
% %         {@{}l | @{\quad}c@{\quad} | c@{\quad} c@{\;} c@{\quad}c@{\;}c@{\;}c@{}}\toprule
% %           & Hardware & \multicolumn{3}{c}{Cost (US\$ per Hr)} \\
% %           & Used &   Single-Server & \algname \\ \midrule
         
% %          % Dex-Net & T4 GPU & 0.53 (1.21x) & 1.04 (2.36x) & 0.44 \\ % spot 0.223

% %          \bottomrule
% %     \end{tabular}
% %     \caption{\textbf{\algname hourly cost saving compared to a Single-Server (one on-demand machine) and Fault Tolerant (FT) (two on-demand machines) deployment on Vision-based Cloud Robotics} \eric{I tend to remove this table: I think the benefit of fault tolerance is clear, and we don't show as much benefit in terms of cost. I think we can do a "one more thing" later in the physical experiment section. }  }
% %     \label{tab:eval:cost}
% % \end{table}


==> tables/exp1results.tex <==
% \begin{table}
%     \centering
%     \footnotesize
%     \begin{tabular}{l l l r r } 
% \toprule
%  & Available & Failure  & Prob. Selecting  & Failure \\ 
% & Machines  & Rate (\%)& Edge(\%) &  Reduction\\
% \midrule
% 1&E-M, E-B    & 26.67 (8/30) & - & 1x, \textbf{2.2x} \\
% 2&E-M, C-W    & 6.67 (2/30)     & 30 (9/30)   &  \textbf{4x}, 1.3x \\
% 3&E-B, C-W     & 10.00 (3/30)    &  6.67 (2/30) & \textbf{5.6x}, 1x\\ 
% 4&E-M, C-E      & 30.00 (9/30)  & 46.67 (14/30) & 1x, \textbf{1.1x} \\ 
% 5&E-B, C-E      & 53.33  (16/30)   &  3.33 (1/30)  &  \textbf{1.1x}, 0.63x \\ 
% 6&E-M, C-W, C-E       &  10.00 (3/30)  & 53.33 (16/30) & 2.7x, 1x, \textbf{3.3x} \\  
% 7&E-B, C-W, C-E       &  6.67 (2/30)  & 0 (0/30)  & \textbf{8.5x}, 1.5x, 5x \\  
% \bottomrule
% \end{tabular}
% \caption{\textbf{Evaluation of \algname in Failure Reduction} \algname selects from available baseline machines and we measure the failure rate (lower the better). \algname matches or surpasses the performance of the best individual machine, reducing the failure rate by up to 8.5 times. By selecting a machine with best latency at a given moment, it can achieve even lower failure rate than up to 1.5 times lower than that of any single machine available. \eric{please help check with the numbers, i did the calculation by hand}}
% \label{tab:eval:exp1:results}
% \vspace{-8pt}
% \end{table}

% \begin{table}
%     \centering
%     \footnotesize
%     \begin{tabular}{l l l l } 
% \toprule
%  Failure & Delay: 20 + 50ms   &  Delay: 20 + 50ms\\ 
%  Rate(\%) & 50\%   Applied     &  100\%  Applied  \\
% \midrule
% Edge1(Delay) &  26.7(8/30)  &  56.7 (17/30)        \\
%     + Edge 2 &  0.0  &  0.0       \\
%     + Cloud(West) &  10.0(3/30)  &  6.7   \\
%     + Cloud(East) &  30.0(9/30)  &  53.3   \\
%     + Cloud(East) + Cloud(West) &  6.7(2/30)   &  10.0   \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Evaluation of \algname in Failure Reduction} \algname selects from available baseline machines and we measure the failure rate (lower the better). \algname matches or surpasses the performance of the best individual machine, reducing the failure rate by up to 8.5 times. By selecting a machine with best latency at a given moment, it can achieve even lower failure rate than up to 1.5 times lower than that of any single machine available.}
% \label{tab:eval:exp1:results}
% \vspace{-8pt}
% \end{table}

\begin{table*}
    \centering
    \setlength{\tabcolsep}{10pt} 
    \renewcommand{\arraystretch}{1.5} % Default value: 1

    \footnotesize
    \begin{tabular}  {l | c | c c c c c c} 
\toprule
 % Failure Rate & Edge 1(Delay)  &  Edge 1(Delay) & Edge 1(Delay) & Edge 1(Delay) \\ 

 Edge 1 (Add Delay) & Edge 1 & Edge 1 & & & \\ 
 Failure Rate (\%)  & Only & + Edge 2     &  + Cloud(W) & + Cloud(E) & + Cloud(W) + Cloud(E)  \\
\hline
 100\% Applied &  56.7\% & 0.0\% & 10.0\% & 30.0\% & \bf{6.7\%}    \\
 % \midrule
    (Failure Reduction) &   & $(\infty)$ & (5.7x) & (1.9x) & \bf{(8.5x)}    \\
\hline
    50\% Applied &  26.7\%  & 0.0\% & \bf{6.7\%} & 53.3\% & 10.0\%  \\
% \midrule
   (Failure Reduction) &   &  ($\infty$) & \bf{(4.0x)} & (0.5x) & (2.7x)  \\
    % + Cloud(East) + Cloud(West) &  6.7(2/30)   &  10.0   \\
\bottomrule
\end{tabular}

\caption{\textbf{When local network was congested, \algname reduced failures:} Upon application of random network delays on Edge \#1, \algname automatically re-route to alternative services, i.e. Edge 2, Cloud(W), Cloud(E).  
Such automatic switching functionality to an alternative, location independent service(s) improves robustness of the system and reduced failure rate (lower the better) of the overall system. 
\algname matches performance of the best individual machine, reducing the failure rate by up to 8.5 times by selecting the best available machine compared to single edge service system under heavy network congestion.
We also showed that \algname enabled flexible yet reliable access to open cloud services via Anycast to reduce failure rate.}
\label{tab:eval:exp1:results}
\vspace{-8pt}
\end{table*}

==> tables/exp1setup.tex <==
\begin{table}
    \centering
    \footnotesize
    \begin{tabular}{ l l l | c c } 
\toprule
 & Candidates & Failure  & Interference  & Interference\\ 
  &          & Rate (\%)& (ms) & Prob. (\%)\\
\midrule
 E-G&Edge (Good)    & 0 (0/30)     & 0     & 0\\
 E-M&Edge (Medium)  & 26.67 (8/30) & $35\pm15$ & 50\\ 
 E-B&Edge (Bad)     & 56.67 (17/30)  & $35\pm15$ & 100\\ 
 C-W&Cloud (West US)     & 10  (3/30)   & -     & -\\ 
 C-E&Cloud (East US)       &  36.67 (10/30)  & -     & -\\ 
\bottomrule
\end{tabular}
\caption{\textbf{Failure Rate and Network Setups of Baseline Machines For Visual Distance Estimation}  The robot controller maintains a direct and stable connection to the Edge server via an Ethernet cable. Interference is introduced with a $35\pm15$ ms network delay, applied at rates of 50\% and 100\% to respectively represent Edge (Medium) and Edge (Bad) conditions. All the robots and edge servers are at California (West US), and the Cloud servers are located at AWS facilities in Oregon (West US) and Ohio (East US). \eric{is 35+-15 the same as 20 + 50? the latter one might be confusing} \marcus{Michael says it's just $50 \pm 0$ ms (no randomness).}
}
\label{tab:eval:exp1:setup}
\vspace{-8pt}
\end{table}

==> tables/time.tex <==

% column: application, experiment time, average uptime, total preemptions 
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{@{}l@{\quad}c@{\quad} c@{\quad}c@{\quad}c@{\quad}c@{\;}c@{\;}c@{}}\toprule
           & Experiment & Preemptions & 1 Response  & 2 Response &  \\
           &  Time (hr) & Experienced & Rate (\%)  & Rate (\%)  \\
         \midrule
        
         YOLO &  25  & 2 & 100 & 75  \\
         SAM  &  25  & 3  & 100  & 75 \\ 
         Dex-Net  &  25  &  3 & 100  & 75 \\ 
         MPT  &  25  & 3  & 100  &75 \\ 
         \bottomrule
    \end{tabular}
    \caption{\textbf{\algname experiment uptime on Cloud Robotics applications} We run all cloud robotics applications with more than 24 hours period and experienced more than 2 preemptions. \algname is able to provide at least one response for all the applications despite the preemptions, and with X \% of receiving responses from multiple servers.\eric{response rate are placeholders}  }
    \label{tab:eval:time}
\end{table}

